MT-Mol:Multi Agent System with Tool-based Reasoning for Molecular Optimization

Large language models (LLMs) have large potential for molecular optimization, as they can gather external chemistry tools and enable collaborative interactions to iteratively refine molecular candidates. However, this potential remains underexplored, particularly in the context of structured reasoning, interpretability, and comprehensive tool-grounded molecular optimization. To address this gap, we introduce MT-Mol, a multi-agent framework for molecular optimization that leverages tool-guided reasoning and role-specialized LLM agents. Our system incorporates comprehensive RDKit tools, categorized into five distinct domains: structural descriptors, electronic and topological features, fragment-based functional groups, molecular representations, and miscellaneous chemical properties. Each category is managed by an expert analyst agent, responsible for extracting task-relevant tools and enabling interpretable, chemically grounded feedback. MT-Mol produces molecules with tool-aligned and stepwise reasoning through the interaction between the analyst agents, a molecule-generating scientist, a reasoning-output verifier, and a reviewer agent. As a result, we show that our framework shows the state-of-the-art performance of the PMO-1K benchmark on 17 out of 23 tasks.

==> tables/task_description.tex <==
\begin{table*}[ht]
\centering
\begin{tabular}{lp{12cm}}
\hline
\textbf{Task Name} & \textbf{Description} \\
\hline
albuterol\_similarity & Generate molecules that resemble the asthma drug albuterol. \\
amlodipine\_mpo & Design molecules similar to amlodipine while matching key drug-like properties. \\
celecoxib\_rediscovery & Recreate molecules highly similar to the anti-inflammatory drug celecoxib. \\
deco\_hop & Replace outer groups of a molecule while keeping the core unchanged. \\
drd2 & Generate molecules predicted to interact with the dopamine D2 receptor. \\
fexofenadine\_mpo & Create fexofenadine-like molecules with similar size, polarity, and flexibility. \\
gsk3b & Find molecules likely to bind to GSK3β, a protein linked to various diseases. \\
isomers\_c7h8n2o2 & Generate isomers with the same formula but different structures. \\
isomers\_c9h10n2o2pf2cl & Generate complex isomers with fluorine, phosphorus, and chlorine atoms. \\
jnk3 & Design molecules predicted to affect the JNK3 protein related to brain and inflammation. \\
median1 & Find molecules that strike a balance across several drug-likeness criteria. \\
median2 & Similar to median1, but with different target property thresholds. \\
mestranol\_similarity & Generate molecules structurally similar to the hormone drug mestranol. \\
osimertinib\_mpo & Create osimertinib-like molecules optimized for cancer treatment properties. \\
perindopril\_mpo & Generate drug-like molecules based on the blood pressure drug perindopril. \\
qed & Maximize an overall drug-likeness score based on multiple chemical properties. \\
ranolazine\_mpo & Design alternatives to ranolazine with similar drug-like behavior. \\
scaffold\_hop & Change the molecule’s core structure while preserving key functions. \\
sitagliptin\_mpo & Generate sitagliptin-like molecules with balanced medicinal properties. \\
thiothixene\_rediscovery & Reproduce the structure of thiothixene, an antipsychotic drug. \\
troglitazone\_rediscovery & Reconstruct the discontinued diabetes drug troglitazone. \\
valsartan\_smarts & Generate molecules containing a key substructure from valsartan. \\
zaleplon\_mpo & Create sleep aid molecules similar to zaleplon, optimized for multiple criteria. \\
\hline
\end{tabular}
\caption{Descriptions of the 23 benchmark tasks used in the PMO framework.}
\label{tab:pmo_tasks}
\end{table*}

